Massive Spikes in LLMs are Bias Vectors: Mechanistic Uncovering and Spike-Free Quantization

Massive activation spikes in Large Language Models (LLMs) severely degrade quantization by stretching dynamic ranges. While prior hypotheses characterize these as high-level scalar biases, we argue that they are merely the scalar intermediates of rigid, structural vector biases in the spike-carrying tokens. We show that these tokens converge to constant vectors after normalization that drive the attention sink and value-state drain mechanisms. We geometrically substantiate this by analyzing the coordination of projection weights: $W_K$ contrastively amplifies the vector, $W_Q$ aligns semantic tokens toward it, and $W_V$ projects it into the spectral null-space. Furthermore, we reveal that the model actively preserves these structural biases against Rotary Positional Embedding (RoPE) perturbations by localizing them in "zones of rotational stability" utilizing low-frequency bands and coherent channel pairs. Leveraging this, we propose INSERTQUANT, a post-training quantization (PTQ) framework that clamps spikes and restores their function via pre-computed template vectors. This renders activations strictly spike-free, enabling robust low-bit quantization with high fidelity. INSERTQUANT achieves parity with state-of-the-art per-tensor quantization methods on LLMs and uniquely generalizes beyond text to other modalities such as ViTs.

==> tables/save_LLM_CSR.tex <==
\begin{table*}[t]
\centering
\scriptsize 
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{2.5pt}

\begin{tabular}{c|cc|cccccccc|cc}
\hline
\textbf{Model} & \textbf{Bits} & \textbf{Method} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{SIQA} & \textbf{HellaS.} & \textbf{OBQA} & \textbf{WinoG.} & \textbf{Wiki} & \textbf{Wiki} \\
 & W-A-KV & & & & & & & & & & \textbf{(2048)} & \textbf{(8192)} \\ \hline

% =========================================================
% MODEL 1: Llama-2-7B
% =========================================================
\multirow{19}{*}{Llama-2-7B} 
 & 16-16-16 & Baseline & 73.78 & 44.97 & 79.33 & 78.67 & 32.91 & 76.15 & 44.00 & 69.38 & 5.47 & - \\ \cdashline{2-13}

 & \multirow{4}{*}{4-8d-8} 
   & RTN         & 71.55 & 44.28 & 75.60 & 78.29 & 32.96 & 74.71 & 41.80 & 68.51 & 5.88 & - \\
 & & QuaRot      & 44.78 & 26.45 & 61.53 & 66.00 & 32.91 & 44.27 & 30.20 & 53.99 & 24.77 & - \\
 & & PrefixQuant & 74.45 & 44.37 & 77.92 & 78.02 & 32.91 & 74.73 & 42.60 & 67.25 & 5.66 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\ \cdashline{2-13}

 & \multirow{4}{*}{4-8d-4} 
   & RTN         & 69.44 & 42.06 & 72.35 & 78.24 & 32.96 & 71.99 & 41.60 & 68.59 & 6.23 & -\\
 & & QuaRot      & 46.34 & 26.28 & 60.89 & 65.45 & 33.11 & 33.75 & 30.60 & 53.12 & 29.42 & - \\
 & & PrefixQuant & 73.82 & 44.80 & 78.17 & 77.91 & 33.11 & 74.68 & 42.80 & 67.01 & 5.72 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\ \cdashline{2-13}

 & \multirow{3}{*}{4-8s-4} 
   & RTN         & 34.01 & 23.29 & 54.07 & 56.64 & 32.24 & 39.09 & 25.60 & 50.67 & 230.03 & - \\
 & & PrefixQuant & 72.90 & 42.83 & 77.55 & 77.64 & 33.01 & 74.29 & 41.20 & 65.75 & 5.79 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\ \cdashline{2-13}

 & \multirow{4}{*}{4-4d-4} 
   & RTN         & 30.18 & 23.38 & 55.54 & 55.17 & 33.62 & 29.45 & 25.40 & 52.09 & 455.40 & - \\
 & & QuaRot      & 37.58 & 24.40 & 58.87 & 60.55 & 33.57 & 31.27 & 28.40 & 50.59 & 40.13 & - \\
 & & PrefixQuant & 70.03 & 43.34 & 75.08 & 76.44 & 33.01 & 54.57 & 42.40 & 65.75 & 6.29 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\ \cdashline{2-13}

 & \multirow{3}{*}{4-4s-4} 
   & RTN         & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\
 & & PrefixQuant & 67.21 & 41.98 & 74.56 & 75.95 & 33.37 & 72.09 & 38.40 & 65.90 & 6.24 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \\ \hline

% =========================================================
% MODEL 2: Llama-3-8B
% =========================================================
\multirow{19}{*}{Llama-3-8B} 
 & 16-16-16 & Baseline & 77.53 & 54.10 & 82.26 & 80.63 & 33.01 & 79.24 & 44.80 & 73.80 & 6.14 & 5.54 \\ \cdashline{2-13}

 & \multirow{4}{*}{4-8d-8} 
   & RTN         & 73.78 & 46.67 & 78.32 & 78.13 & 32.91 & 77,24 & 45.80 & 71.51 & 7.58 & 6.88 \\
 & & QuaRot      & 69.82 & 43.43 & 72.02 & 75.03 & 33.32 & 70.95 & 39.60 & 70.24 & 9.27 & 8.10 \\
 & & PrefixQuant & 76.89 & 49.91 & 76.18 & 79.43 & 32.96 & 77.36 & 41.40 & 70.88 & 6.81 & 6.13 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}

 & \multirow{4}{*}{4-8d-4} 
   & RTN         & 70.58 & 43.60 & 74.59 & 74.81 & 32.91 & 74.52 & 41.60 & 69.93 & 8.76 & 7.87  \\
 & & QuaRot      & 68.73 & 41.13 & 73.94 & 74.21 & 33.62 & 69.00 & 73.94 & 68.67 & 9.55 & 8.38 \\
 & & PrefixQuant & 78.78 & 49.91 & 78.38 & 79.82 & 32.86 & 76.81 & 41.60 & 69.61 & 6.95 & 6.26 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}

 & \multirow{3}{*}{4-8s-4} 
   & RTN         & 43.14 & 23.46 & 47.46 & 60.55 & 32.96 & 39.88 & 29.60 & 55.80 & 79.24 & 65.89 \\
 & & PrefixQuant & 70.33 & 40.96 & 74.25 & 76.06 & 32.91 & 72.27 & 36.20 & 65.04 & 7.01 & 6.33 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}

 & \multirow{4}{*}{4-4d-4} 
   & RTN         & 35.77 & 23.21 & 49.79 & 57.45 & 33.27 & 35.58 & 28.60 & 49.33 & 253.13 & 245.95 \\
 & & QuaRot      & 53.62 & 31.40 & 51.99 & 66.65 & 33.37 & 58.45 & 33.40 & 56.35 & 17.41 & 14.83 \\
 & & PrefixQuant & 71.38 & 44.54 & 69.51 & 76.44 & 32.96 & 73.48 & 39.20 & 64.33 & 8.19 & 7.35 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}

 & \multirow{3}{*}{4-4s-4} 
   & RTN         & 26.77 & 23.63 & 43.09 & 50.44 & 36.28 & 26.44 & 25.80 & 50.75 & 3401.22 & 3241.54 \\
 & & PrefixQuant & 69.65 & 41.04 & 75.26 & 73.88 & 32.86 & 71.66 & 40.00 & 62.12 & 8.38 & 7.54 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

% =========================================================
% MODEL 3: Mistral-7B
% =========================================================
\multirow{19}{*}{Mistral-7B} & 16-16-16 & Baseline & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-8d-8} & RTN & 77.82 & 51.28 & 81.93 & 81.18 & 32.91 & 79.20 & 46.00 & 73.48 & 5.84 & 5.17 \\
 & & QuaRot & 68.48 & 44.03 & 80.28 & 78.45 & 32.91 & 75.51 & 41.20 & 69.77 & 6.63 & 5.80 \\
 & & PrefixQuant & 77.57 & 51.54 & 82.29 & 80.58 & 32.91 & 80.06 & 43.20 & 71.51 & 5.52 & 4.91 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-8d-4} & RTN & 78.20 & 51.02 & 81.90 & 79.87 & 32.91 & 78.14 & 47.20 & 71.59 & 6.07 & 5.42 \\
 & & QuaRot & 67.68 & 43.86 & 80.37 & 78.02 & 32.96 & 74.92 & 41.20 & 69.61 & 6.82 & 5.98 \\
 & & PrefixQuant & 77.10 & 50.68 & 81.96 & 81.18 & 32.91 & 79.73 & 42.80 & 71.51 & 5.57 & 4.96 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{3}{*}{4-8s-4} & RTN & 48.19 & 28.84 & 51.80 & 61.21 & 33.42 & 36.19 & 29.80 & 55.88 & 268.19 & 612.80 \\
 & & PrefixQuant & 77.02 & 49.74 & 82.84 & 80.69 & 32.91 & 79.33 & 43.60 & 71.82 & 5.62 & 5.01 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-4d-4} & RTN & 59.13 & 38.05 & 66.21 & 72.47 & 33.06 & 65.10 & 37.20 & 58.80 & 16.48 & 16.48 \\
 & & QuaRot & 63.17 & 38.74 & 75.35 & 75.73 & 33.01 & 69.69 & 38.00 & 64.33 & 7.95 & 6.92 \\
 & & PrefixQuant & 75.08 & 47.10 & 78.13 & 79.05 & 32.86 & 78.35 & 43.60 & 67.01 & 5.92 & 5.27 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{3}{*}{4-4s-4} & RTN & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant & 75.08 & 46.50 & 80.18 & 79.38 & 32.91 & 76.93 & 43.20 & 68.98 & 5.92 & 5.29 \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

\end{tabular}
\caption{TODO (Preliminary version) Comprehensive performance comparison on 8 CSR tasks and 2 Wiki perplexity benchmarks.}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize 
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{2.5pt}

\begin{tabular}{c|cc|cccccccc|cc}
\hline
\textbf{Model} & \textbf{Bits} & \textbf{Method} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{SIQA} & \textbf{HellaS.} & \textbf{OBQA} & \textbf{WinoG.} & \textbf{Wiki} & \textbf{Wiki} \\
 & W-A-KV & & & & & & & & & & \textbf{(2048)} & \textbf{(8192)} \\ \hline

\multirow{19}{*}{Llama-2-13B} & 16-16-16 & Baseline & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-8d-8} & RTN & 74.07 & 46.67 & 78.93 & 79.65 & 31.78 & 76.63 & 43.80 & 67.96 & 5.32 & - \\
 & & QuaRot & 75.76 & 46.59 & 79.69 & 79.11 & 33.06 & 74.25 & 44.80 & 70.80 & 6.03 & - \\
 & & PrefixQuant & 77.44 & 48.29 & 79.66 & 79.92 & 32.96 & 77.68 & 45.60 & 72.77 & 5.02 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-8d-4} & RTN & 72.05 & 45.39 & 76.57 & 78.73 & 33.27 & 75.19 & 42.60 & 67.40 & 5.54 & - \\
 & & QuaRot & 74.58 & 45.65 & 79.51 & 78.89 & 32.96 & 73.68 & 43.60 & 70.09 & 6.07 & - \\
 & & PrefixQuant & 77.86 & 47.87 & 80.18 & 79.71 & 33.47 & 77.35 & 45.00 & 73.01 & 5.07 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{3}{*}{4-8s-4} & RTN & 51.73 & 32.76 & 61.74 & 64.74 & 34.49 & 52.68 & 30.20 & 51.46 & 92.17 & - \\
 & & PrefixQuant & 77.82 & 47.53 & 80.12 & 79.60 & 33.67 & 77.40 & 44.60 & 71.43 & 5.10 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{4}{*}{4-4d-4} & RTN & 25.88 & 25.85 & 38.75 & 49.51 & 32.29 & 25.95 & 24.80 & 50.20 & 1888.81 & - \\
 & & QuaRot & 70.54 & 39.16 & 70.12 & 75.35 & 33.32 & 67.36 & 38.00 & 64.33 & 7.63 & - \\
 & & PrefixQuant & 75.59 & 47.87 & 79.05 & 78.40 & 32.50 & 75.99 & 43.60 & 71.19 & 5.52 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-13}
 & \multirow{3}{*}{4-4s-4} & RTN & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant & 76.60 & 46.93 & 79.94 & 79.38 & 33.01 & 76.51 & 43.40 & 71.59 & 5.53 & - \\
 & & InsertQuant & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

\end{tabular}
\caption{TODO}
\end{table*}

==> tables/tab_complete_LLM_CSR_results.tex <==
\begin{table*}[t]
\centering
\scriptsize 
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{2.5pt}

\caption{\textbf{Detailed results for LLM quantization.} We report per-task accuracy on common-sense reasoning benchmarks: \textit{acc} for BoolQ, SIQA, and WinoGrande, and \textit{acc\_norm} for ARC-e, ARC-c, PIQA, HellaSwag, and OBQA. \textbf{Avg. Acc.} denotes the mean across tasks. We also report WikiText2 perplexity at context lengths 2048 and 8192 (lower is better). ``d'' and ``s'' indicate per-token dynamic and per-tensor static activation quantization, respectively. All methods are evaluated without fine-tuning and use the same calibration setting. LLaMA2-7b does not natively support 8192 sequence lengths and is excluded from those evaluations.}
\label{tab:full_result}

\begin{tabular}{c|cc|ccccccccc|cc}
\hline
\textbf{Model} & \textbf{Bits} & \textbf{Method} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{SIQA} & \textbf{HellaS.} & \textbf{OBQA} & \textbf{WinoG.} & \textbf{Avg. Acc.} & \textbf{Wiki} & \textbf{Wiki} \\
 & W-A-KV & & & & & & & & & & & \textbf{(2048)} & \textbf{(8192)} \\ \hline

% =========================================================
% MODEL 1: Llama-2-7B
% =========================================================
\multirow{19}{*}{Llama-2-7B} & 16-16-16 & Baseline & 73.78 & 44.97 & 79.33 & 78.67 & 32.91 & 76.15 & 44.00 & 69.38 & 62.40 & 5.47 & - \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-8} & RTN & 71.80 & 44.28 & 76.27 & 78.02 & 32.80 & 74.55 & 42.00 & 68.35 & 61.01 & 5.88 & - \\
 & & QuaRot-RTN & 44.23 & 26.28 & 56.79 & 64.15 & 33.73 & 41.66 & 29.40 & 54.46 & 43.84 & 30.19 & - \\
 & & PrefixQuant & 73.99 & 43.86 & 77.74 & 78.07 & 33.01 & 75.33 & 43.00 & 69.69 & 61.84 & 5.66 & - \\
 & & InsertQuant & 72.98 & 43.34 & 77.77 & 79.05 & 32.96 & 74.77 & 43.00 & 68.75 & 61.58 & 5.68 & - \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-4} & RTN & 70.37 & 43.09 & 75.02 & 78.24 & 33.01 & 73.56 & 41.00 & 67.48 & 60.22 & 6.04 & - \\
 & & QuaRot-RTN & 44.23 & 26.28 & 56.79 & 64.15 & 33.73 & 41.66 & 29.40 & 54.46 & 43.84 & 30.19 & - \\
 & & PrefixQuant & 72.98 & 43.94 & 77.83 & 77.86 & 33.11 & 75.24 & 43.40 & 68.27 & 61.58 & 5.70 & - \\
 & & InsertQuant & 73.19 & 42.83 & 77.03 & 78.89 & 33.21 & 74.47 & 43.40 & 68.67 & 61.46 & 5.73 & - \\ \cdashline{2-14}
 & \multirow{3}{*}{4-8s-4} & RTN & 39.18 & 27.73 & 56.09 & 60.17 & 33.16 & 43.11 & 28.00 & 53.75 & 42.65 & 30.84 & - \\
 & & PrefixQuant & 72.94 & 43.09 & 77.71 & 77.86 & 32.75 & 74.87 & 42.60 & 68.75 & 61.32 & 5.77 & - \\
 & & InsertQuant & 72.90 & 42.58 & 77.19 & 78.35 & 33.11 & 73.97 & 43.20 & 68.27 & 61.19 & 5.84 & - \\ \cdashline{2-14}
 & \multirow{4}{*}{4-4d-4} & RTN & 27.90 & 24.57 & 56.21 & 53.21 & 33.67 & 29.97 & 26.60 & 49.33 & 37.68 & 439 & - \\
 & & QuaRot-RTN & 34.97 & 23.29 & 58.23 & 59.14 & 32.50 & 36.73 & 27.00 & 51.22 & 40.39 & 45.69 & - \\
 & & PrefixQuant & 70.24 & 43.17 & 74.59 & 75.73 & 33.47 & 74.38 & 42.80 & 66.85 & 60.15 & 6.27 & - \\
 & & InsertQuant & 69.74 & 42.83 & 73.58 & 76.99 & 33.11 & 72.92 & 41.00 & 66.14 & 59.54 & 6.30 & - \\ \cdashline{2-14}
 & \multirow{3}{*}{4-4s-4} & RTN & 26.22 & 28.41 & 43.76 & 48.37 & 32.29 & 25.43 & 26.40 & 48.15 & 34.88 & 7072 & - \\
 & & PrefixQuant & 71.38 & 42.83 & 75.96 & 77.69 & 32.75 & 73.57 & 40.60 & 67.72 & 60.31 & 6.22 & - \\
 & & InsertQuant & 70.20 & 43.17 & 74.92 & 77.09 & 33.01 & 72.38 & 41.20 & 65.19 & 59.65 & 6.30 & - \\ \hline


% =========================================================
% MODEL 2: Llama-3-8B
% =========================================================
\multirow{19}{*}{Llama-3-8B} & 16-16-16 & Baseline & 77.53 & 54.10 & 82.26 & 80.63 & 33.01 & 79.24 & 44.80 & 73.80 & 65.67 & 6.14 & 5.54 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-8} & RTN & 74.49 & 47.10 & 80.24 & 78.02 & 32.91 & 77.22 & 46.00 & 72.14 & 63.51 & 7.58 & 6.89 \\
 & & QuaRot-RTN & 69.02 & 42.75 & 66.76 & 74.59 & 33.27 & 69.97 & 40.00 & 70.88 & 58.40 & 9.45 & 8.32 \\
 & & PrefixQuant & 76.81 & 52.65 & 80.40 & 79.11 & 32.96 & 77.91 & 43.80 & 72.61 & 64.53 & 6.81 & 6.14 \\
 & & InsertQuant & 76.94 & 52.22 & 80.46 & 79.71 & 33.32 & 78.17 & 43.20 & 71.90 & 64.49 & 6.83 & 6.14 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-4} & RTN & 74.03 & 46.76 & 73.64 & 75.90 & 32.91 & 75.89 & 43.40 & 70.64 & 61.65 & 8.08 & 7.39 \\
 & & QuaRot-RTN & 69.02 & 42.75 & 66.76 & 74.59 & 33.27 & 69.97 & 40.00 & 70.88 & 58.40 & 9.45 & 8.32 \\
 & & PrefixQuant & 75.63 & 52.82 & 79.63 & 79.54 & 32.91 & 77.75 & 43.00 & 70.72 & 64.00 & 6.91 & 6.23 \\
 & & InsertQuant & 75.76 & 51.02 & 80.64 & 79.11 & 33.01 & 77.53 & 43.60 & 72.45 & 64.14 & 6.92 & 6.23 \\ \cdashline{2-14}
 & \multirow{3}{*}{4-8s-4} & RTN & 42.93 & 26.11 & 55.44 & 62.02 & 32.55 & 42.49 & 29.80 & 53.75 & 43.14 & 64.25 & 61.09 \\
 & & PrefixQuant & 75.93 & 51.62 & 79.88 & 78.89 & 32.96 & 77.28 & 42.80 & 71.67 & 63.88 & 7.00 & 6.31 \\
 & & InsertQuant & 74.79 & 50.09 & 78.96 & 78.73 & 33.01 & 77.28 & 45.20 & 71.43 & 63.68 & 7.07 & 6.38 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-4d-4} & RTN & 37.37 & 25.00 & 50.55 & 56.80 & 32.50 & 37.84 & 29.80 & 49.01 & 39.86 & 167.37 & 189 \\
 & & QuaRot-RTN & 57.28 & 32.08 & 58.10 & 66.27 & 32.80 & 58.52 & 35.40 & 58.01 & 49.81 & 17.91 & 14.88 \\
 & & PrefixQuant & 70.37 & 46.16 & 74.19 & 76.55 & 32.70 & 75.17 & 38.60 & 66.85 & 60.07 & 8.13 & 7.30 \\
 & & InsertQuant & 71.09 & 45.05 & 71.28 & 75.35 & 32.86 & 75.57 & 41.60 & 65.98 & 59.85 & 8.19 & 7.34 \\ \cdashline{2-14}
 & \multirow{3}{*}{4-4s-4} & RTN & 25.34 & 23.98 & 39.30 & 51.36 & 31.88 & 26.38 & 25.00 & 53.04 & 34.53 & 5647 & 4970 \\
 & & PrefixQuant & 72.94 & 45.39 & 76.27 & 77.64 & 33.11 & 75.23 & 41.40 & 67.64 & 61.20 & 8.35 & 7.51 \\
 & & InsertQuant & 72.31 & 46.59 & 69.14 & 75.90 & 32.55 & 74.20 & 39.60 & 65.75 & 59.50 & 8.91 & 8.12 \\ \hline


% =========================================================
% MODEL 3: Mistral-7B
% =========================================================
\multirow{19}{*}{Mistral-7B} & 16-16-16 & Baseline & 80.05 & 54.35 & 83.70 & 81.99 & 32.91 & 80.69 & 47.20 & 74.03 & 66.87 & 5.32 & 4.75 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-8} & RTN & 79.04 & 51.54 & 82.08 & 80.52 & 32.91 & 79.27 & 46.80 & 72.69 & 65.61 & 6.48 & 5.17 \\
 & & QuaRot-RTN & 68.06 & 42.83 & 79.91 & 77.58 & 32.91 & 75.08 & 41.00 & 71.03 & 61.05 & 6.75 & 5.94 \\
 & & PrefixQuant & 78.96 & 52.73 & 82.48 & 80.85 & 32.91 & 79.98 & 44.00 & 72.38 & 65.53 & 5.52 & 4.91 \\
 & & InsertQuant & 76.81 & 49.91 & 83.82 & 80.96 & 32.91 & 77.41 & 45.40 & 72.93 & 65.02 & 5.72 & 5.04 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-8d-4} & RTN & 78.79 & 50.60 & 82.35 & 80.85 & 32.91 & 78.56 & 45.80 & 71.82 & 65.21 & 6.45 & 5.42 \\
 & & QuaRot-RTN & 68.06 & 42.83 & 79.91 & 77.58 & 32.91 & 75.08 & 41.00 & 71.03 & 61.05 & 6.75 & 5.94 \\
 & & PrefixQuant & 79.08 & 52.13 & 82.81 & 80.79 & 32.91 & 79.91 & 43.80 & 71.82 & 65.41 & 5.56 & 4.95 \\
 & & InsertQuant & 75.88 & 49.15 & 83.82 & 80.85 & 32.96 & 77.12 & 44.80 & 72.14 & 64.59 & 5.76 & 5.10 \\ \cdashline{2-14}
 & \multirow{3}{*}{4-8s-4} & RTN & 49.37 & 27.90 & 50.18 & 60.39 & 32.09 & 36.20 & 29.60 & 54.30 & 42.50 & 243 & 612 \\
 & & PrefixQuant & 78.28 & 51.37 & 82.60 & 80.41 & 32.91 & 79.71 & 43.80 & 72.45 & 65.19 & 5.60 & 4.99 \\
 & & InsertQuant & 75.93 & 48.81 & 82.94 & 81.07 & 32.86 & 76.87 & 44.40 & 72.38 & 64.40 & 5.79 & 5.14 \\ \cdashline{2-14}
 & \multirow{4}{*}{4-4d-4} & RTN & 45.33 & 28.16 & 52.29 & 59.25 & 32.45 & 40.71 & 27.00 & 50.51 & 41.96 & 356 & 16.48 \\
 & & QuaRot-RTN & 63.59 & 38.65 & 74.50 & 74.27 & 32.80 & 68.59 & 39.40 & 63.77 & 56.95 & 8.10 & 6.93 \\
 & & PrefixQuant & 76.68 & 48.63 & 78.93 & 79.82 & 32.91 & 78.58 & 42.80 & 68.43 & 63.35 & 5.90 & 5.25 \\
 & & InsertQuant & 72.94 & 47.78 & 79.88 & 78.67 & 32.96 & 74.26 & 42.20 & 68.43 & 62.14 & 6.24 & 5.51 \\ \cdashline{2-14}
 & \multirow{3}{*}{4-4s-4} & RTN & 26.22 & 29.10 & 40.89 & 49.46 & 31.83 & 26.13 & 23.80 & 48.86 & 34.53 & INF & INF \\
 & & PrefixQuant & 77.53 & 49.49 & 82.08 & 79.27 & 32.86 & 78.89 & 43.20 & 70.17 & 64.18 & 5.90 & 5.26 \\
 & & InsertQuant & 73.27 & 47.78 & 81.77 & 79.16 & 32.96 & 74.94 & 44.00 & 70.72 & 63.08 & 6.14 & 5.50 \\ \hline


\end{tabular}
\end{table*}


==> tables/tab_complete_LLM_OLLMv1_results.tex <==
\begin{table*}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{5pt} % Adjusted spacing for 9 columns

\begin{tabular}{c|cc|cccccc}
\hline
\textbf{Model} & \textbf{Bits} & \textbf{Method} & \textbf{ARC-c} & \textbf{HellaS.} & \textbf{MMLU} & \textbf{TruthfulQA} & \textbf{WinoG.} & \textbf{GSM8K} \\
 & W-A-KV & & & & & & & \\ \hline

% =========================================================
% MODEL 1: Llama-2-7B
% =========================================================
\multirow{21}{*}{Llama-2-7B} 
 & 16-16-16 & Baseline    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}
 
 % Group: 4-8d-8
 & \multirow{5}{*}{4-8d-8} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 % Group: 4-8d-4
 & \multirow{5}{*}{4-8d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 % Group: 4-4d-4
 & \multirow{5}{*}{4-4d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 % Group: 4-4s-4
 & \multirow{5}{*}{4-4s-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

% =========================================================
% MODEL 2: Llama-3-8B
% =========================================================
\multirow{21}{*}{Llama-3-8B} 
 & 16-16-16 & Baseline    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}
 
 & \multirow{5}{*}{4-8d-8} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-8d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-4d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-4s-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

% =========================================================
% MODEL 3: Mistral-7B
% =========================================================
\multirow{21}{*}{Mistral-7B} 
 & 16-16-16 & Baseline    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}
 
 & \multirow{5}{*}{4-8d-8} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-8d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-4d-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \cdashline{2-9}

 & \multirow{5}{*}{4-4s-4} 
   & RTN            & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & QuaRot         & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & SpinQuant      & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & PrefixQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\
 & & InsertQuant    & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline

\end{tabular}
\caption{TODO. (Preliminary version) Comparison of accuracy on Huggingface Open LLM leader-board versions 1 (OLLMv1).}
\end{table*}

